Streamforce: outsourcing access control enforcement for stream data to the clouds

As tremendous amount of data being generated everyday from human activity and from devices equipped with sensing capabilities, cloud computing emerges as a scalable and cost-effective platform to store and manage the data. While benefits of cloud computing are numerous, security concerns arising when data and computation are outsourced to a third party still hinder the complete movement to the cloud. In this paper, we focus on the problem of data privacy on the cloud, particularly on access controls over stream data. The nature of stream data and the complexity of sharing data make access control a more challenging issue than in traditional archival databases. We present Streamforce - a system allowing data owners to securely outsource their data to the cloud. The owner specifies fine-grained policies which are enforced by the cloud. The latter performs most of the heavy computations, while learning nothing about the data. To this end, we employ a number of encryption schemes, including deterministic encryption, proxy-based attribute based encryption and sliding-window encryption. In Streamforce, access control policies are modeled as secure continuous queries, which entails minimal changes to existing stream processing engines, and allows for easy expression of a wide-range of policies. In particular, Streamforce comes with a number of secure query operators including Map, Filter, Join and Aggregate. Finally, we implement Streamforce over an open source stream processing engine (Esper) and evaluate its performance on a cloud platform. The results demonstrate practical performance for many real-world applications, and although the security overhead is visible, Streamforce is highly scalable.

==> protocol.tex <==
\section{The Protocols}
\label{sec:protocol}
\subsection{Overview}
Our protocols for both trigger and sliding window policies consist of 3 phases, as illustrated
in Figure~\ref{fig:context}. First, the data owner and user negotiate an access control
policy which can be either a trigger or sliding
window policy (negotiation phase). Next, the data owner encrypts its data and sends
it to the cloud (outsourcing phase). Upon receiving
the ciphertexts, the cloud performs transformation on the ciphertexts and forwards the results
to the authorized users (relaying phase). The users receive messages from the cloud and decrypt them to obtain
the plaintext data.

A naive approach would be for the data owner to generate one encryption key for each policy,
share this key to the authorized users, and encrypt the data using this key. This does not
scale for two reasons. First, the amount of duplicated data that must be encrypted grows
linearly with the number of policies. Second, for a sliding window
policy $\pi(\alpha,\beta)$, the owner has to transform the data locally and update the
encrypted version to the cloud. This process must be done for every combination of $\alpha$ and
$\beta$.

In our protocol, there is only encrypted copy of the data stored at the cloud for the
trigger policies, and up-to $w$ copies for sliding window policies where $w$ is the number of
unique window sizes. To this end, we make use of three important cryptographic primitives: attribute-based
encryption (ABE), proxy re-encryption (PRE) and additive homomorphic encryption (AHE). ABE is
used to enforce threshold conditions specified in trigger policies, as well as the
condition on the starting index in sliding window policies. PRE is used by the cloud to
transform ABE ciphertexts to simpler ciphertexts that can be decrypted by users. The aims of
this transformation is to relieve the users from carrying out expensive operations involving
ABE. For sliding window policies, AHE enables the cloud to compute the encrypted aggregates of
the data windows over the encrypted text without breaking data privacy.

\subsection{Cryptographic Primitives}
\subsubsection{Attribute Based Encryption.}
Attribute-Based Encryption (ABE) schemes produce ciphertexts that
can only be decrypted if a set of attributes satisfies certain
conditions (or policies). Two types of ABE exists: key-policy
ABE~\cite{goyal06} (KP-ABE) and ciphertext-policy
ABE~\cite{bethencourt07} (CP-ABE). In both cases, a policy is
expressed as an access structure over a set of attributes. For
example, if the policy is defined as the predicate $T = a_1 \,
\wedge \, (a_2 \vee a_3)$, then $T(\{a_1\}) = T(\{a_2,a_3\}) =
\mbox{false}$, $T(\{a_1,a_2\}) = T(\{a_1,a_3\}) = \mbox{true}$. The
plaintext can be recovered only if evaluating the policy over the
given attributes returns true.
%\begin{figure}
%\centering
%\includegraphics[scale=0.45]{figures/abe_numerical.pdf}
%\caption{An example of access structure expressing the policy $(a \cup b) \cap x \leq 11$}
%\label{fig:accessStructure}
%\end{figure}

In KP-ABE, the message $m$ is encrypted with a set of attributes $A$
and an access structure $T$ is embedded in a decryption key. In
CP-ABE, $T$ is embedded within the ciphertext and the user is given
a set of attribute $A$. In both cases, decryption will succeed and
return $m$ if $T(A) = \mbox{true}$. KP-ABE and CP-ABE are based on
secret sharing schemes that generate shares in a way that the
original secret will only be reconstructed if a certain access
structure is satisfied. Constructions of KP-ABE and CP-ABE for any
linear secret sharing scheme (modelled as a span program) are
described in~\cite{goyal06,bethencourt07}. In practice, the schemes
rely on threshold tree structures for secret sharing, in which
non-leaf nodes are threshold gates (AND and OR).

We adopt KP-ABE in our work, which is more suitable than CP-ABE,
because the attributes are based on the plaintext message (the key
value $k$). Although KP-ABE and CP-ABE are similar and in some cases
can be used interchangeably, the former is more data-centric
(concerning the question of who gets access to the given data),
whereas the latter is more user-centric (concerning the question of
which data the given user has access to). For the trigger policy
$\tau(\theta,op)$ we encrypt $(k_i,v_i)$ using KP-ABE with $k_i$ as
the attribute and $k \ op \ \theta = \mbox{true}$ as the policy.
Similarly, for the sliding window policy $\pi(\alpha,\beta)$, we
encrypt $(k_i,v_i)$ using $k_i$ as the attribute and $k \geq \alpha$
as the policy.

Since the policies involve arithmetic comparison, we make use of the \emph{bag-of-bits} method
that translates an integer into a set of attributes. For example, with $64$-bit integers,
an attribute $3$ can be mapped to $\{x..x1x, x..x1\}$, and the policy $k \geq 11$ can be mapped
into $(ge2exp4 \,\vee \, ge2exp8 \,\vee\, ge2exp16 \,\vee\, ge2exp32) \vee (x..1xxx \,\wedge\,
(x..1xx \, \vee \, (x..x1x \,\wedge\, x..xx1)))$ where $ge2expm$ is an attribute representing
values greater than or equal to $2^m$. It can be seen that a policy involving equality
condition often involves more attributes than a policy with an inequality condition.

\subsubsection{Proxy Re-Encryption.}
A Proxy Re-Encryption scheme (PRE)~\cite{blaze98} enables a third-party to transform one
ciphertext to another without learning the plaintext. Using a \emph{transformation key} $K_{U
\to V}$ it can convert $c = \enc(K_U,m)$ to $c' = \enc(K_V,m)$ which can be decrypted with
$K_V$, without learning $m$. Traditional PRE schemes have been used for distributed file
systems, in a way that saves the data owner from having different copies of the same data for
different users. In this work, we extend a recent proxy-based ABE scheme~\cite{green11} which
can transform a KP-ABE ciphertext into a Elgamal-like ciphertext whenever the access structure
is satisfied. This scheme has the benefit of traditional PRE schemes, and it relieves users
from expensive computations involving ABE.

\subsubsection{Additive Homomorphic Encryption.}
Sliding window policies require that authorized users have access to the averages of data values
within non-overlapping windows. To allow for such an aggregate operation over
ciphertexts, the encryption scheme must be additively homomorphic, i.e.  $\enc(K,m_1) \oplus
\enc(K,m_2) = \enc(K,m_1+m_2)$ for an operator $\oplus$. Paillier~\cite{paillier99}
is one of such schemes, which is based on composite residuosity classes of group
$\mathbb{Z}_{N^2}$ where $N$ is at least 1024-bit.

In this work, we use an Elgamal-like encryption scheme to achieve
additive homomorphism, which can also be integrated with ABE.
Essentially, consider a multiplicative group $\mathbb{Z}_p$ with generator
$g$. For $m \in \mathbb{Z}_p$, $K$ and $r$ as random values of
$\mathbb{Z}_p$, then $\enc(K,m) = (g^r, g^m.g^{r.K})$. The
homomorphic property holds, because $\enc(K,m_1).\enc(K,m_2) =
\enc(K,m_1+m_2)$. The drawback of this scheme is that decryption
requires finding the discrete logarithm of $g^m$ in base $g$. As in
other works using a similar scheme~\cite{cramer97,zhong07,ugus09},
we assume that the plaintext domain is finite and small so that
discrete logarithms can be computed by brute-force~\cite{pollard78}
or even pre-computed and cached. For many types of applications
where data values belong to a small set (such that temperature
values), this is a reasonable assumption. Note that the security is
not compromised due to the mapping of $g^m$ to $m$, which merely acts as an
additional layer used to achieve homomorphism.

To prevent a user from learning the individual values constituting a
window, we introduce a blind factor into the ciphertext, which can
only be removed when a proper number of ciphertexts are put
together. Suppose the windows are of size $2$, the owner generates
$\delta_1,\delta_2$ randomly and give $\sigma = \delta_1+\delta_2$
to the user. The ciphertext $c_1 = (g^{r_1},g^m.g^{r_1+\delta_1+K})$
and $c_2 = (g^{r_2},g^{m_2}.g^{r_2+\delta_2+K})$ cannot be decrypted
individually, since $\delta_1$ and $\delta_2$ are unknown to the
user. However, $c_1.c_2 = (X = g^{r_1+r_2}, Y =
g^{m_1+m_2}.g^{K(r_1+r_2+\delta_1+\delta_2)})$ can be decrypted by
computing $g^{m_1+m_2} = \frac{Y}{X^K.g^{\sigma.K}}$ and recovering
$m_1+m_2$ by taking its discrete logarithm. In our protocol, the
user only needs to know $\sigma$ for the starting window, with which
the unblind factors for the subsequent windows can be efficiently
computed.

\subsection{Protocol for Sliding Window Policies}
\begin{figure}
    \centering
    \includegraphics[scale=0.45]{figures/chart.pdf}
    \caption{High-level protocol}
    \label{fig:highLevelProt}
\end{figure}
Figure~\ref{fig:highLevelProt} illustrates the high-level protocol for sliding window policies.
In the negotiation phase, data owner and user agrees on the sliding window parameters
$\alpha,\beta$. The owner generates an access tree $T$ for the condition $k \geq \alpha$, a
transformation key $TK$ and a decryption key $K$ for the user. It sends $(\alpha,\beta,TK,K)$
to the user and $(\alpha, \beta,TK)$ to the cloud. For every tuple $(k_i,v_i)$, the owner
encrypts $v_i$ using KP-ABE with attribute $k_i$.  Each tuple is encrypted $\omega$ times, each
for a different window size $\beta$ and using a different blind factor. During the relaying
phase, the cloud selects ciphertexts whose attribute is greater or equal to $\alpha$,
and transforms them using $TK$ into other ciphertexts that can be decrypted with another key
$K'$ $(K \neq K')$. Every $\beta$ of the transformed ciphertexts are used as inputs to the
\texttt{ComputeSum} function which produces an encrypted sum value which can be decrypted
using $K$.

Our protocol relies on the properties of \emph{bilinear maps} for security. Let $G,G_1$
be two multiplicative groups of prime order $p$, $g$ be the generator of $G$. $e:G
\times G \to G_1$ is a bilinear map if it is efficiently computable, $e(u^a,v^b) =
e(u,v)^{a.b}$ for $u,v \in G$ and   $e(g,g) \neq 1$. Given random group elements $g^a,
g^b, g^c$, it is difficult to compute $e(g,g)^{abc}$ (Computational Bilinear Diffie-Hellman
Assumption). Also, it is difficult to distinguish $e(g,g)^{abc}$ from a random element
$e(g,g)^z$ (Decisional Bilinear Diffie-Hellman Assumption).

\textbf{Negotiation phase.}
During setup, all parties agree on a security parameter $\lambda$.  Let $U$ be the attribute
universe, i.e. $U = \{x..x0, x..x1, x..0x, ...\}$. The owner chooses a master secret value $y
\in \mathbb{Z}_p$, and other secret $t_1, t_2,.. t_{|U|}$. For every window size $\beta$, it
generates a set of random values $R = \{r_0, r_1,..,r_{\beta-1}\}$. The public key contains
$e(g,g)^y, g^{t_1}, g^{t_2}, .., g^{t_{|U|}}$.

Let $u$ be an user with a sliding policy $\pi(\alpha,\beta)$. The owner generates a
random value $z_u \in \mathbb{Z}_p$. Next, the policy $k \geq \alpha$ is converted into an
access tree whose leaves are the bag-of-bit representation of $k$, as explained
in~\cite{goyal06}. Every non-leaf node is a threshold gate: an AND node is a 2-out-of-2 threshold
gate, an OR node is a 1-out-of-2 gate. This tree is used to share the master secret $y$. For a
node $x$ with threshold $d_x$, choose a random polynomial $q_x$ of degree $d_x-1$ (so
that $x_d$ points are needed to reconstruct the polynomial). For the root node, set $q_r(0) =
y$. For any other node, set $q_x(0) = q_{parent(x)}(index(x))$ where $q_{parent(x)}$ is the
polynomial of $x$'s parent and $index(x)$ is the node index. The leaf node $x$
associated with an attribute $i$ is given the value $D_x = g^{\frac{q_x(0)}{z_u.t_i}}$.

For the policy $\pi(\alpha,\beta)$, the owner computes:
\[
\sigma(\alpha,\beta) =  \sum_{j=0}^{\beta-1} 2^{\lceil (\alpha+j)/\beta \rceil}R[\alpha+j \ mod \ \beta]
\]
Finally, the user is sent
\[(\alpha, \beta, \{D_x\}, (z_u, \sigma(\alpha,\beta)))
\]
where $\{D_x\}$ and $(z_u,\sigma(\alpha,\beta))$ are the
transformation and user decryption keys respectively.

\textbf{Outsourcing phase.}
To encrypt $(k,v) \in D$, the data owner first translates $k$ into bag-of-bit attributes $B_k$.
Next, it chooses a random value $s_k \in \mathbb{Z}_p$ and computes $E'_i = g^{t_i.s_k}$ for all
attribute $i \in B_k$.  It also computes:
\[
E(k,v) = g^{v+2^{\lceil k/\beta \rceil}.R[k \ mod \ \beta]}.e(g,g)^{y.s_k}
\]
Finally, the following ciphertext is forwarded to the cloud:
\[
c_k = (k, B_k, E(k,v), \{E'_i\})
\]


\textbf{Relaying phase.}
The transformation proceeds recursively as follows. When $x$ is a leaf node associated with attribute $i$:
\[
    \trans(x) = \left\{
                \begin{array}{l}
                e(D_x,E'_i) = e(g,g)^{\frac{s_k.q_x(0)}{z_u}}\ \text{when $i \in B_k$}\\
                \bot \qquad \text{otherwise}
                \end{array}
                \right.
\]

When $x$ is a non-leaf node, we call $\trans(w)$ for all $w$ that are $x$'s children.
Let $\Delta_{i,S}(x) = \prod_{j \in S, j\neq i}\frac{x-j}{i-j}$ be the Lagrange
coefficient for an element $i \in \mathbb{Z}_p$ and $S \subseteq \mathbb{Z}_p$.
Let $F_w$ be the output of $\trans(w)$, and $S_x$ be the set of $x$'s children such
that $F_w \neq \bot$. If $S_x = \emptyset$, return $\bot$. Otherwise:
\begin{align*}
    F_x & = \trans(x)\\
    & = \prod_{w \in S_x}F_w^{\Delta_{index(w),S'_x}(0)} \ \text{where
$S'_x=\{index(w) \,|\, w \in S_x\}$}\\
%   & = \prod_{w \in S_x}(e(g,h)^{y.q_w(0)/z_u})^{\Delta_{index(w),S'_x}(0)}\\
%   & = \prod_{w \in
%S_x}(e(g,h)^{y.q_{parent(w)}(index(w))/z_u})^{\Delta_{index(w),S'_x}(0)} \\
%   & = \prod_{w \in S_x}e(g,h)^{y.q_x(0)/z_u.\Delta_{index(w),S'_x}(0)} \\
    & = e(g,g)^{s_k.q_x(0)/z_u}
\end{align*}
By calling $\trans$ on the root node of the access tree, we obtain $\trans(root_k) =
e(g,g)^{y.s_k/z_u}$. Let $C_k = (E(k,v), \trans(root_k))$. For the $i^{th}$ window, the
cloud has to gather the full set of $\mathbb{C} = \{C_k, C_{k+1}, .., C_{k+\beta-1}\}$ for $k = \alpha+i.\beta$. Then, it
executes \texttt{ComputeSum} as follows:
\begin{align*}
(E_1, E_2) &= \texttt{ComputeSum}(\mathbb{C}) = \prod_{j=0}^{\beta-1} C_{k+j}\\
&= (\prod_{j=0}^{\beta-1} E(k+j,
v_{k+j}), \prod_{j=0}^{\beta-1} \trans(root_{k+j}))
\end{align*}
and sends $(i = \frac{k-\alpha}{\beta}, E_1, E_2)$ to the user.

Having received this message from the cloud, the user computes:
\begin{align*}
w_i &= \frac{E_1}{E_2^{z_u}} =
\frac{E(k,v).E(k+1,v_1)..E(k+\beta-1,v_{\beta-1})}{(e(g,g)^{y.s_k/z_u}..e(g,g)^{y.s_{k+\beta-1}/z_u})^{z_u}}\\
&=\frac{g^{(v_k+..+v_{k+\beta-1})+2^i.\sigma(\alpha,\beta)}.e(g,g)^{(s_k+..+s_{k+\beta-1}).y/z_u}}{(e(g,g)^{(s_k+..+s_{k+\beta-1}).y/z_u})^{z_u}}\\
&=g^{(v_k+..+v_{k+\beta-1})+2^i.\sigma(\alpha,\beta)}
\end{align*}
Finally, the average is computed as:
\[
avg_i = \frac{\mbox{discreteLog}(\frac{w_i}{g^{2^i.\sigma(\alpha,\beta)}})}{\beta} =
\frac{v_k+..+v_{k+\beta-1}}{\beta}
\]

\vspace{0.3cm}

\subsection{Protocol for Trigger Policy}
The protocol for trigger policies is very similar to that for sliding window. Its main
differences are that the access policies  may involve other conditions besides  $\geq$ as in
sliding window, and that no blind factor is needed since authorized users can access individual
data tuples.

During the negotiation phase, the owner create the public key containing $e(g,g)^y,
g^{t_1}, g^{t_2},.., g^{t_{|U|}}$ as before. Next, the access structure for the policy $k \, op
\, \theta$ is constructed. The
transformation key contains $\{D_x\}$ for all leaf node $x$, and the user decryption key is
$z_u$. During the outsourcing phase, a ciphertext sent to the cloud is generated in the same
way as with sliding window policy, except for $E(k,v) = g^v.e(g,g)^{y.s_k}$. During
transformation, the cloud computes $\trans(root_k) = e(g,g)^{y.s_k/z_u}$ as before and
sends $C_k = (E(k,v), \trans(root_k))$ to the user, who decrypts it by taking the discrete
logarithm of
$g^v = \frac{E(k,v)}{(\trans(root_k))^{z_u}}$.

\vspace{0.3cm}

\subsection{Discussions}
\textbf{Security.}
The  protocols described above provide data privacy with respect to the cloud, because we
use an encryption scheme which is an extension of the proxy-based ABE scheme proposed
in~\cite{green11}.  As shown in \cite{green11}, the scheme is Replayable-CCA (or RCCA) secure.
Our encryption is secure in the standard model (as opposed to security in random oracle model),
since we use the small-universe construction of ABE.

The access control property for trigger policies hold as a result of
ABE. For sliding window policies, we now discuss an informal proof
showing that unauthorized access is not possible. Particularly, we
need to show that an user given access according to a policy
$\pi(\alpha,\beta)$ cannot decrypt values belonging to other
policies $\pi(\alpha',\beta')$ where $\alpha' < \alpha$, $\beta' <
\beta$, $\alpha' \neq \alpha \ mod \ \beta$ or $\beta' \neq 0 \ mod
\ \beta$. Since the ciphertext is encrypted with the attribute $k$
and the policy embedded in the transformation key requires $k \geq
\alpha$, the $\trans$ operation will fail for $k < \alpha$. Thus,
the user is prevented from learning the values in
$\pi(\alpha',\beta')$ for $\alpha'<\alpha$. From
$\sigma(\alpha,\beta)$, one can infer the value
$\sigma(\alpha',\beta)$ for $\alpha'>\alpha$ and $\alpha' = \alpha \
mod \ \beta$, since $\sigma(\alpha',\beta) =
2^{\alpha'/\alpha}.\sigma(\alpha,\beta)$. However, for $\alpha' \neq
\alpha \ mod \ \beta$, deriving $\sigma(\alpha', \beta')$ from
$\sigma(\alpha,\beta)$ is not possible as it requires knowing the
sum of a subset of $R$. Therefore, the user cannot recover the
plaintext because the unblind factors are incorrect. This similarly
holds when $\beta' < \beta$ or $\beta' \neq 0 \ mod \ \beta$,
because computing the blind factors $\sigma(\alpha',\beta')$ in
these cases requires knowing individual values of $R$.

\textbf{Scalability.} The most expensive cryptographic operations
are exponentiations and pairings. The latter are done only by the
cloud during transformation. The number of pairings is proportional
to the size of the access tree.  Notice that the access tree is
likely to be smaller for a sliding window policy than for a trigger
policy, as there is a smaller number of attributes involved in
constructing $k > x$ than in constructing $k = x$. Without the
cloud, the user will have to perform these pairings themselves.
Instead, in our protocol, the user only performs simple operations
such as inversion, multiplication, and only one exponentiation.
Having to find discrete logarithm during decryption is a potential
bottleneck. But as discussed earlier, we assume the data value
domain is known and finite, hence the user may pre-compute the
discrete logarithm, thus reducing this problem into a simple table
look-up. If $m$ is the maximum value that $v$ can take, the look-up
table has the size of $m$ for trigger policies, and $b.m$ for
sliding policies where $b$ is the maximum window size.

The data owner's computations are during the negotiation phase and
the outsourcing phase. Public and master key are generated only
once, hence the cost will amortize over time. Generation of
transformation keys is done once per policy. Compared to data
encryption during the outsourcing phase, this operation is much less
frequent and can be considered as a constant. Thus to say, the
overall setup cost is a one-off cost which amortizes over time.
During the outsourcing phase, the owner performs one encryption per
data value for trigger policies, and $w$ encryptions for sliding
window policies ($w$ being the number of window sizes). The cost per
encryption is roughly the same for both trigger and sliding
policies, and is dominated by the cost of $2+b$ exponentiations.

There are overheads incurred when storing the ciphertexts in the cloud. First, ABE encryption
introduces overheads that are proportional to the number of attributes per ciphertext. These
overhead are constant in our protocol, because the number of attributes is fixed at $b$.
Second, the data owner may wish to support sliding window policies of different window sizes,
which entails storing multiple ciphertexts for the same data value at the cloud. However, when
encrypting $(k,v)$ for different values of $\beta$ only $E(k,v)$ will be different. As a
result, the overhead is limited to $w.||G||$ where $||G||$ is the number of bits per group element.

